Beamforming in MISO Systems: Empirical Results and EVM-based Analysis

We present an analytical, simulation, and experimental-based study of beamforming Multiple Input Single Output (MISO) systems. We analyze the performance of beamforming MISO systems taking into account implementation complexity and effects of imperfect channel estimate, delayed feedback, real Radio Frequency (RF) hardware, and imperfect timing synchronization. Our results show that efficient implementation of codebook-based beamforming MISO systems with good performance is feasible in the presence of channel and implementation-induced imperfections. As part of our study we develop a framework for Average Error Vector Magnitude Squared (AEVMS)-based analysis of beamforming MISO systems which facilitates comparison of analytical, simulation, and experimental results on the same scale. In addition, AEVMS allows fair comparison of experimental results obtained from different wireless testbeds. We derive novel expressions for the AEVMS of beamforming MISO systems and show how the AEVMS relates to important system characteristics like the diversity gain, coding gain, and error floor.

==> 1-Introduction.tex <==
\section{Introduction}
% The very first letter is a 2 line initial drop letter followed
% by the rest of the first word in caps.
% 
% form to use if the first word consists of a single letter:
% \IEEEPARstart{A}{demo} file is ....
% 
% form to use if you need the single drop letter followed by
% normal text (unknown if ever used by IEEE):
% \IEEEPARstart{A}{}demo file is ....
% 
% Some journals put the first two words in caps:
% \IEEEPARstart{T}{his demo} file is ....
% 
% Here we have the typical use of a "T" for an initial drop letter
% and "HIS" in caps to complete the first word.

%%%%%
% ME commented out
%\IEEEPARstart{T}{his} demo file is intended to serve as a ``starter file''
%for IEEE journal papers produced under \LaTeX\ using
%IEEEtran.cls version 1.7 and later.
% You must have at least 2 lines in the paragraph with the drop letter
% (should never be an issue)
%I wish you the best of success.

% ME commented out

\IEEEPARstart{S}{tandards} for next generation wireless communications have considered the use beamforming Multiple Input Single Output (MISO) systems with codebook-based feedback because these systems can potentially achieve same diversity order and larger coding gain compared to non-feedback systems like space-time codes \cite{Embrace,HeathOverview,HeathGrassm,Kiran}. Recently, the performance of beamforming MISO systems has been analyzed taking into account errors in the channel estimate, and/or feedback delay \cite{RaoBER,YMaJournal,SK,YMaDelayICE,BFLetters}, and noise in the feedback channel \cite{Index}. However, these results do not take into account effects of non-ideal RF processing, imperfect timing synchronization or consider implementation complexity.

In this paper we evaluate the performance of codebook based beamforming MISO systems taking into account implementation complexity and the presence of channel and implementation-induced imperfections. Specifically, we consider channel-induced imperfections which are due to channel estimation errors and feedback delay and we consider implementation-induced imperfections which are a result of imperfect timing synchronization and non-ideal RF processing, Automatic Gain Control (AGC), Analog to Digital Converters (ADCs), and Digital to Analog Converters (DACs). Since not all imperfections can be modeled tractably, especially implementation-induced imperfections, we adopt a mixed approach of analytical, simulation, and experimental evaluation. Analytical and simulation results presented in this paper take into account channel-induced imperfections but do not take into account implementation-induced imperfections because these imperfections are difficult to model in a tractable way. Thus, we complement these results with experimental results which do take into account both channel and implementation-induced imperfections. This mixed approach provides a more complete picture of expected performance.

Inclusion of experimental evaluation poses a unique challenge in the choice of evaluation metric. Common metrics like Bit Error Rate (BER) or Symbol Error Rate (SER) are usually analyzed as a function of the average Energy per Symbol to Noise ratio ($E_s/N_o$) or average Energy per Bit to Noise ratio ($E_b/N_0$). However, when real hardware is used for evaluation of wireless systems, getting an accurate measurement of the noise or the $E_s/N_o$ or $E_b/N_o$ proves problematic because the noise can be non-linear, both multiplicative and additive, and may depend on radio settings and characteristics of the received signal. In contrast, the Average Error Vector Magnitude Squared (AEVMS), a metric commonly used in test equipment, can be easily measured since it is computed at the input of the demodulator. As a result, we propose to use the AEVMS as a metric for performance analysis. This leads to the natural question regarding the relationship between AEVMS and $E_s/N_o$ or $E_b/N_o$.

Our first contribution is a framework for AEVMS-based analysis of beamforming MISO systems. Although the Error Vector Magnitude (EVM) and EVM-based metrics are heavily used in industry for testing of wireless devices \cite{EfficientEVM,Agilent}, there is very little theory behind the use of EVM for performance analysis. Some previous work can be found in \cite{AG2,AG1,EVMHP,EVMIslam,EfficientEVM,Agilent}  but no previous work has analyzed the performance of beamforming MISO systems using an EVM related metric. We present simulation, analytical, and experimental results that show how the AEVMS relates to the $E_s/N_o$, BER, diversity gain, coding gain, and error floor. Since BER and AEVMS are quantities that can be directly measured, using these two metrics allows a straightforward comparison of analytical, simulation, and experimental results on the \emph{same} scale. Furthermore, using metrics like BER and AEVMS facilitates comparison of results obtained with different wireless testbeds because these metrics are usually easy to measure in any testbed. We show that BER vs. (1/AEVMS) results can be used to analyze the diversity gain of a system. We also show that coding gain and error floors can be analyzed by looking at the AEVMS performance as a function of the $E_s/N_o$ or an $E_s/N_o$ related metric like the signal power. 

Our second contribution is the performance analysis of beamforming MISO systems as a function of the amount of training used for channel estimation. In particular, we consider two different beamforming systems: a 1 round (1R) system which uses only 1 round of training and a 1.5 round (1.5R) system which uses 1.5 rounds of training (we use the terminology for multi round training defined in \cite{AshuMultiRound}). We present novel results on the AVEMS vs. $E_s/N_o$ performance of the 1R and 1.5R systems in the presence of channel estimation errors and feedback delay. These results show that in the presence of feedback delay, 1.5 rounds of training eliminate the error floor that is present when only one round of training is used. Taking into account noisy channel estimate and feedback delay, work in \cite{RaoBER} analyzed the BER and SER for a 1R system and work in \cite{YMaDelayICE} analyzed the capacity of a 1.5R system. However, previous work does not include comparison and AEVMS-based analysis of error floor of 1R and 1.5R systems in the presence of imperfect channel estimate and feedback delay. 

Our third contribution is an experimental evaluation which demonstrates that efficient implementation of codebook based beamforming MISO systems with good performance is feasible in the presence of channel and implementation-induced imperfections. We show that beamforming codebooks proposed in \cite{HeathKerdock,MyMilcom}, which are known to facilitate efficient implementation and storage, can achieve performance close to infinite feedback (infinite codebook size) using only few feedback bits (small codebook size) and have better performance than a space-time code system like Alamouti. This result had not been demonstrated in the presence of channel and implementation-induced imperfections. Experimental results for beamforming systems have been reported in \cite{FPGATests,Valenzuela} but these works have not considered codebook based feedback. We also consider the tradeoff between implementation complexity and performance in WiMAX compliant systems. Our experimental results demonstrate that the Mixed Codebook scheme for WiMAX compliant systems proposed in \cite{MyMilcom,MyAsilomar} has good performance and simplifies implementation of beamforming in WiMAX compliant systems.


The rest of the paper is organized as follows. Section \ref{sec:SystemModelAndBeamforming} describes the channel model and implementation requirements for the beamforming systems that are considered in this paper. The framework for AEVMS-based analysis of beamforming MISO systems is presented in Section \ref{sec:AEVSMderivation}, this section also presents error floor analysis of 1R and 1.5R systems. Section \ref{sec:ExperimentSetupAndResults} describes the experimental setup and presents experiment results. Conclusions are presented in Section \ref{sec:Conclusions}.

==> 5-Conclusions.tex <==
\section{Conclusion}
\label{sec:Conclusions}
We presented a comprehensive study of beamforming MISO systems. We presented simulation, analytical, and experimental results, and analyzed implementation requirements and effect of channel and implementation-iduced imperfections. Our results show that, using EGB codebooks, it is feasible to efficiently implement codebook-based beamforming MISO systems that have good performance. We also showed that the Mixed Codebook scheme simplifies the implementation complexity of WiMAX beamforming systems. Finally, we showed that the AEVMS is a relevant metric for performance analysis of beamforming MISO systems which facilitates comparison between theoretical and experimental results and can also facilitate comparison between experimental results obtained with different wireless testbeds.

